Climate Risk and Corporate Value: Evidence from Temperature Bins and Panel Regression

In empirical research, this article uses daily climate data provided by the National Oceanic and Atmospheric Administration (NOAA) of the United States to construct a temperature box with a range of 5\( ^\circ\text{C} \), focusing on analyzing the impact of extreme high temperatures (\( >30^\circ\text{C} \)) and extreme low temperatures (\( \le -10^\circ\text{C} \)) on the asset value of enterprises. The results based on a panel regression model show that extreme high and low temperatures can significantly reduce the asset value of enterprises. In the robustness test, this article used lagged climate data for testing, and the results still showed that extreme high temperatures had a significant negative impact on the asset value of enterprises, verifying the reliability of the benchmark regression results. In-depth heterogeneity analysis shows that in the process of addressing climate risks, companies exhibit significant differentiation based on different ownership types and industry characteristics. According to research, state-owned enterprises are relatively less affected by extreme weather due to their resource advantages and policy preferences. In addition, foreign-funded enterprises demonstrate a high level of risk resistance due to their strong management efficiency and supply chain control capabilities. In the manufacturing sector, heavy industries such as steel and communication manufacturing are particularly affected by the negative effects of extreme weather, which fully demonstrates that these industries face more severe challenges when dealing with extreme weather conditions.

==> configs/preamble.tex <==
%
% --- inline annotations
%
\usepackage[dvipsnames]{xcolor}
\newcommand{\red}[1]{{\color{black}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}




==> sections/discussion.tex <==
\section{Discussion and Conclusion}

In a nutshell, our image generation approach is a sequence model operated on a tokenized latent space \cite{Chen2020,Esser2021,Ramesh2021}. But unlike previous methods that are based on vector-quantized tokenizers (\eg, variants of VQ-VAE  \cite{Oord2017,Esser2021}), we aim to use continuous-valued tokenizers (\eg, \cite{Rombach2022}). We propose Diffusion Loss that makes sequence models compatible with continuous-valued tokens.

\subsection{Rethinking Discrete-Valued Tokens}
\label{sec:discrete}

To begin with, we revisit the roles of discrete-valued tokens in autoregressive generation models.  Denote as $x$ the ground-truth token to be predicted at the next position. With a discrete tokenizer,  $x$ can be represented as an integer: $0 \leq x < K $, with a vocabulary size $K$.
The autoregressive model produces a continuous-valued $D$-dim vector $z \in \mathbb{R}^D $, which is then projected by a $K$-way classifier matrix $W \in \mathbb{R}^{K{\times}D}$. Conceptually, this formulation models a \textit{categorical probability distribution} in the form of $p(x | z) = \text{softmax}({W}{z})$.

\subsection{Diffusion Loss}

Consider a continuous-valued vector $x \in \mathbb{R}^d$, which denotes the ground-truth token to be predicted at the next position.
The autoregressive model produces a vector $z \in \mathbb{R}^D$ at this position. Our goal is to model a probability distribution of $x$ conditioned on $z$, that is, $p(x|z)$. The loss function and sampler can be defined following the diffusion models \cite{Ho2020,Nichol2021,Dhariwal2021}, described next.


\paragraph{Loss function}. Following \cite{Ho2020,Nichol2021,Dhariwal2021}, the loss function of an underlying probability distribution $p(x|z)$ can be formulated as a denoising criterion:

\paragraph{Sampler}. At inference time, it is required to draw samples from the distribution $p(x|z)$. Sampling is done via a reverse diffusion procedure \cite{Ho2020}: 

Here $\delta$ is sampled from the Gaussian distribution $\mathcal{N}( \mathbf{0}, \mathbf{I})$ and $\sigma_t$ is the noise level at time step $t$. Starting with $x_{T} \sim \mathcal{N}( \mathbf{0}, \mathbf{I})$, this procedure produces a sample $x_{0}$ such that $x_{0} \sim p(x|z)$ \cite{Ho2020}.

\subsection{Diffusion Loss for Autoregressive Models}

We can rewrite this formulation in two parts. We first produce a conditioning vector $z^i$ by a network (\eg, Transformer \cite{Vaswani2017}) operating on previous tokens: $z^i = f(x^1, ..., x^{i-1})$. Then, we model the probability of the next token by $p(x^i | z^i)$. Diffusion Loss in Eqn.~(\ref{eq:denoise}) can be applied on $p(x^i | z^i)$. The gradient is backpropagated to $z^i$ for updating the parameters of $f(\cdot)$.


\begin{align}
	\text{Cvalue}_{it} &= \alpha + \sum_{j=1}^{9} \beta^j \, \text{Tembin}_{it}^j + \phi X_{it} + \delta_i + \tau_t + \varepsilon_{it} \\
	\text{Cvalue}_{it} &= \alpha + \sum_{j=1}^{9} \beta^j \, (L^1 \text{Tembin})_{it}^j + \phi (L^1 X)_{it} + \delta_i + \tau_t + \varepsilon_{it}
\end{align}

==> sections/experiments.tex <==
% \newpage 
\section{Experiments}

%##################################################################################################
\begin{table}[t]
	\caption{
		\textbf{Descriptive Statistics}
	}
	
	\label{Descriptive Statistics}
	\vspace{.5em}
	\begin{minipage}{1.0\linewidth}{\begin{center}
				\tablestyle{6pt}{1.05}
				\begin{tabular}{lccccc}
					\hline
					\textbf{VARIABLES} & mean & standard deviation & minimum & maximum & number of observations\\
					\hline
					cvalue & 0.3559 & 0.2071 & 0.0130 & 0.9290 & 1,381,908 \\
					wind & 5.7906 & 1.5136 & 0.5888 & 15.5043 & 1,381,908 \\
					sea & 1015.75 & 1.7188 & 991.1 & 1056 & 1,381,908 \\
					visb & 8.7805 & 1.8305 & 3.5175 & 18.6411 & 1,381,908 \\
					25$\sim$30℃ & 52.6142 & 34.9701 & 0 & 189 & 1,381,908 \\
					$>$30℃ & 0.7608 & 1.8884 & 0 & 60 & 1,381,908 \\
					\hline
				\end{tabular}%
			\end{center}
	}\end{minipage}
	\vspace{-1em}
\end{table}
%##################################################################################################


%##################################################################################################
\begin{table}[t]
\caption{
\textbf{Benchmark Regression Results}
}

\label{Benchmark Regression Result}
\vspace{.5em}
\begin{minipage}{1.0\linewidth}{\begin{center}
\tablestyle{6pt}{1.05}
\begin{tabular}{lcccc}
	\hline
	\textbf{VARIABLES} & cvalue (1) & cvalue (2) & cvalue (3) &  cvalue (4)\\
	\hline
	$\leq -10^\circ$C  & -0.000631*** & -0.000319*** & -0.000631*** & -0.000319** \\
	& (8.10e-05)   & (8.24e-05)   & (0.000149)   & (0.000145)   \\
	-10$\sim$-5$^\circ$C & -0.000304*** & -6.22e-05    & -0.000304**  & -6.22e-05    \\
	& (7.22e-05)   & (7.35e-05)   & (0.000135)   & (0.000129)   \\
	-5$\sim$0$^\circ$C  & -0.000110**  & 0.000135**   & -0.000110    & 0.000135     \\
	& (5.57e-05)   & (5.69e-05)   & (0.000110)   & (0.000107)   \\
	0$\sim$5$^\circ$C   & -0.000112*** & 7.74e-05*    & -0.000112    & 7.74e-05     \\
	& (4.32e-05)   & (4.43e-05)   & (8.98e-05)   & (8.58e-05)   \\
	5$\sim$10$^\circ$C  & -1.12e-05    & 0.000175***  & -1.12e-05    & 0.000175**   \\
	& (3.61e-05)   & (3.67e-05)   & (7.51e-05)   & (7.27e-05)   \\
	15$\sim$20$^\circ$C & 5.15e-05     & 7.79e-05**   & 5.15e-05     & 7.79e-05     \\
	& (3.14e-05)   & (3.16e-05)   & (6.65e-05)   & (6.40e-05)   \\
	20$\sim$25$^\circ$C & 7.69e-05***  & 5.88e-05**   & 7.69e-05     & 5.88e-05     \\
	& (2.56e-05)   & (2.57e-05)   & (5.20e-05)   & (4.94e-05)   \\
	25$\sim$30$^\circ$C & -0.000192*** & -0.000163*** & -0.000192**  & -0.000163**  \\
	& (3.04e-05)   & (3.17e-05)   & (9.64e-05)   & (7.77e-05)   \\
	$>$30$^\circ$C     & -0.000190    & -0.000506*** & -0.000190    & -0.000506*   \\
	& (0.000124)   & (0.000126)   & (0.000236)   & (0.000260)   \\
	wind               &              & -0.0129***   &              & -0.0129***   \\
	&              & (0.000419)   &              & (0.00151)    \\
	sea                &              & -0.00148***  &              & -0.00148*    \\
	&              & (0.000372)   &              & (0.000823)   \\
	visb               &              & 0.00187***   &              & 0.00187      \\
	&              & (0.000407)   &              & (0.00174)    \\
	Constant           & 0.365***     & 1.904***     & 0.365***     & 1.904**      \\
	& (0.00715)    & (0.378)      & (0.0158)     & (0.837)      \\
	Controls           & N            & Y            & N            & Y            \\
	Year FE            & Y            & Y            & Y            & Y            \\
	Firm FE            & Y            & Y            & Y            & Y            \\
	Year-by-city FE    & N            & N            & Y            & Y            \\
	Observations       & 1,381,908    & 1,381,908    & 1,381,908    & 1,381,908    \\
	R-squared          & 0.142        & 0.142        & 0.142        & 0.142        \\
	\hline
\end{tabular}%
\caption*{\footnotesize Standard errors in parentheses. *** p$<$0.01, ** p$<$0.05, * p$<$0.1}
\end{center}
}\end{minipage}
\vspace{-1em}
\end{table}
%##################################################################################################

We experiment on ImageNet \cite{deng2009imagenet} at a resolution of 256$\times$256.
We evaluate FID \cite{Heusel2017} and IS \cite{Salimans2016}, and provide Precision and Recall as references following common practice \cite{Dhariwal2021}.
We follow the evaluation suite provided by \cite{Dhariwal2021}.

\subsection{Properties of Diffusion Loss}

\paragraph{Diffusion Loss \vs Cross-entropy Loss}. We first compare continuous-valued tokens with Diffusion Loss and standard discrete-valued tokens with cross-entropy loss (Table~\ref{tab:diffloss_vs_crossent}). 
For fair comparisons, the tokenizers (``VQ-16" and ``KL-16") are both downloaded from the LDM codebase \cite{Rombach2022}.
These are popularly used tokenizers (\eg, \cite{Esser2021,Rombach2022,Peebles2023}).

The comparisons are in four variants of AR/MAR.
As shown in Table~\ref{tab:diffloss_vs_crossent}, Diffusion Loss consistently outperforms the cross-entropy counterpart in all cases. Specifically, in MAR (\eg, the default), using Diffusion Loss can reduce FID by relatively \app50\%-60\%. This is because the continuous-valued \mbox{KL-16} has smaller compression loss than VQ-16 (discussed next in Table~\ref{tab:tokenizer}), and also because a diffusion process models distributions more effectively than categorical ones.

In the following ablations, unless specified, we follow the ``default" MAR setting in Table~\ref{tab:diffloss_vs_crossent}.

%##################################################################################################
\begin{figure}[t]
	\centering
	\hspace{-1.5em}
	\includegraphics[width=0.8\linewidth]{figures/Benchmark regression coefficient plot}
	\caption{\textbf{Benchmark regression coefficient plot}}
	\label{Benchmark regression coefficient plot}
	\vspace{.5em}
\end{figure}

%##################################################################################################

\paragraph{Flexibility of Diffusion Loss}.
One significant advantage of Diffusion Loss is its flexibility with various tokenizers. We compare several publicly available tokenizers in Table~\ref{tab:tokenizer}.

Diffusion Loss can be easily used even given a VQ tokenizer. We simply treat the continuous-valued latent before the VQ layer as the tokens. This variant gives us 7.82 FID (w/o CFG), compared favorably with 8.79 FID (Table~\ref{tab:diffloss_vs_crossent}) of cross-entropy loss using the \textit{same} VQ tokenizer. This suggests the better capability of diffusion for modeling distributions.

This variant also enables us to compare the VQ-16 and KL-16 tokenizers using \textit{the same loss}. As shown in Table~\ref{tab:tokenizer}, VQ-16 has a much \textit{worse} reconstruction FID (rFID) than KL-16, which consequently leads to a much worse generation FID (\eg, 7.82 \vs 3.50 in Table~\ref{tab:tokenizer}).

Interestingly, Diffusion Loss also enables us to use tokenizers with \textit{mismatched} strides. In Table~\ref{tab:tokenizer}, we study a KL-8 tokenizer whose stride is 8 and output sequence length is 32$\times$32. Without increasing the sequence length of the generator, we group 2$\times$2 tokens into a new token. Despite the mismatch, we are able to obtain decent results, \eg, KL-8 gives us 2.05 FID, \vs KL-16's 1.98 FID.
Further, this property allows us to investigate other tokenizers, \eg, Consistency Decoder \cite{OpenAI2024}, a non-VQ tokenizer of a different architecture/stride designed for different goals.

For comprehensiveness, we also train a KL-16 tokenizer on ImageNet using the code of \cite{Rombach2022}, noting that the original KL-16 in \cite{Rombach2022} was trained on OpenImages \cite{Krasin2017}. The comparison is in the last row of Table~\ref{tab:tokenizer}. We use this tokenizer in the following explorations.

%##################################################################################################
\begin{figure}[t]
	\centering
	\hspace{-1.5em}
	\includegraphics[width=0.8\textwidth]{figures/Industry type heterogeneity analysis (screening model)}
	\caption{\textbf{Industry type heterogeneity analysis (screening model)}}
	\label{Industry type heterogeneity analysis (screening model)}
	\vspace{-1.5em}
\end{figure}
%##################################################################################################

\paragraph{Denoising MLP in Diffusion Loss}. We investigate the denoising MLP in Table~\ref{tab:mlp}.
Even a very small MLP (\eg, 2M) can lead to competitive results. As expected, increasing the MLP width helps improve the generation quality;
we have explored increasing the depth and had similar observations.
Note that our default MLP size (1024 width, 21M) adds only \app5\% extra parameters to the MAR-L model. 
During inference, the diffusion sampler has a decent cost of \app10\% overall running time. Increasing the MLP width has negligible extra cost in our implementation (Table~\ref{tab:mlp}), partially because the main overhead is not about computation but memory communication.

\textbf{Sampling Steps of Diffusion Loss}. Our diffusion process follows the common practice of DDPM \cite{Ho2020,Dhariwal2021}: we train with a 1000-step noise schedule but inference with fewer steps. Figure~\ref{fig:diff_steps} shows that using 100 diffusion steps at inference is sufficient to achieve a strong generation quality.

\textbf{Temperature of Diffusion Loss}. 
In the case of cross-entropy loss, the temperature is of central importance. Diffusion Loss also offers a temperature counterpart for controlling the diversity and fidelity. Figure~\ref{fig:tau} shows the influence of the temperature $\tau$ in the diffusion sampler (see Sec.~\ref{sec:diffloss}) at inference time. The temperature $\tau$ plays an important role in our models, similar to the observations on cross-entropy-based counterparts (note that the cross-entropy results in Table~\ref{tab:diffloss_vs_crossent} are with their optimal temperatures).

%##################################################################################################
\begin{table}[t]
	\caption{
		\textbf{Robustness Test}
	}
	
	\label{Robustness Test}
	\vspace{.5em}
	\begin{minipage}{1.0\linewidth}{\begin{center}
				\tablestyle{6pt}{1.05}
				\begin{tabular}{lcccc}
					\hline
					\textbf{VARIABLES} & cvalue (1) & cvalue (2) & cvalue (3) &  cvalue (4)\\
					\hline
					L25$\sim$30℃ & -0.000218*** & -0.000171*** & -0.000218** & -0.000171* \\
					& (3.61e-05)   & (3.69e-05)   & (9.77e-05)  & (8.83e-05)  \\
					$>$30℃      & -0.000259**  & -0.000549*** & -0.000259   & -0.000549*** \\
					& (0.000115)   & (0.000116)   & (0.000192)  & (0.000208)  \\
					Lwind       &              & -0.0124***   &             & -0.0124***  \\
					&             & (0.000427)   &             & (0.00143)   \\
					Lsea        &              & -0.000854**  &             & -0.000854   \\
					&             & (0.000365)   &             & (0.000730)  \\
					Lvisb       &              & -0.000654    &             & -0.000654   \\
					&             & (0.000399)   &             & (0.00143)   \\
					Constant    & 0.359***     & 1.292***     & 0.359***    & 1.292*      \\
					& (0.00755)    & (0.371)      & (0.0173)    & (0.738)     \\
					Controls           & N    & Y    & N    & Y \\
					Year FE            & Y    & Y    & Y    & Y \\
					Firm FE            & Y    & Y    & Y    & Y \\
					Year-by-city FE    & N    & N    & Y    & Y \\
					Observations       & 1,358,119 & 1,358,064 & 1,358,119 & 1,358,064 \\
					R-squared          & 0.142 & 0.143 & 0.142 & 0.143 \\
					\hline
				\end{tabular}%
				\caption*{\footnotesize Standard errors in parentheses. *** p$<$0.01, ** p$<$0.05, * p$<$0.1}
			\end{center}
	}\end{minipage}
	\vspace{-1em}
\end{table}
%##################################################################################################


\subsection{Properties of Generalized Autoregressive Models}

\paragraph{From AR to MAR}. Table~\ref{tab:diffloss_vs_crossent} is also a comparison on the AR/MAR variants, which we discuss next.
First, replacing the raster order in AR with \textit{random} order has a significant gain, \eg, reducing FID from 19.23 to 13.07 (w/o CFG). Next, replacing the causal attention with the \textit{bidirectional} counterpart leads to another massive gain, \eg, reducing FID from 13.07 to 3.43 (w/o CFG).

The random-order, bidirectional AR is essentially a form of MAR that predicts one token at a time. Predicting \textit{multiple} tokens (`$>$1') at each step can effectively reduce the number of autoregressive steps. In Table~\ref{tab:diffloss_vs_crossent}, we show that the MAR variant with 64 steps slightly trades off generation quality. A more comprehensive trade-off comparison is discussed next.

\paragraph{Speed/accuracy Trade-off}. Following MaskGIT \cite{Chang2022}, our MAR enjoys the flexibility of predicting multiple tokens at a time. This is controlled by the number of autoregressive steps at inference time. Figure~\ref{fig:speed} plots the speed/accuracy trade-off. MAR has a better trade-off than its AR counterpart, noting that AR is with the efficient kv-cache.

With Diffusion Loss, MAR also shows a favorable trade-off in comparison with the recently popular Diffusion Transformer (DiT) \cite{Peebles2023}. As a latent diffusion model, DiT models the interdependence across \textit{all} tokens by the diffusion process. The speed/accuracy trade-off of DiT is mainly controlled by its diffusion steps. Unlike our diffusion process on a small MLP, the diffusion process of DiT involves the \textit{entire} Transformer architecture. Our method is more accurate and faster. 
Notably, our method can generate at a rate of $<$ 0.3 second per image with a strong FID of $<$ 2.0.

\vspace{-.2em}

%##################################################################################################

\begin{table}[t]
	\caption{\textbf{Ownership Heterogeneity Analysis}}
	\label{Ownership Heterogeneity Analysis}
	\vspace{.5em}
	\begin{center}
		\resizebox{\textwidth}{!}{ % 缩放到页面宽度
			\begin{tabular}{lccccc}
				\hline
				\textbf{VARIABLES} & Private Enterprises & State-owned Enterprises & Collective Enterprises & Mixed Enterprises & Foreign-owned Enterprises)\\
				\hline
				$\leq$-10℃  & -0.000479*** & -0.000345 & -0.000183 & -0.000465*** & 0.000153 \\
				& (0.000145)   & (0.000219) & (0.000218) & (0.000167) & (0.000355) \\
				-10$\sim$-5℃ & -0.000155    & 0.000408** & -9.47e-06  & -0.000313** & 8.75e-05 \\
				& (0.000128)   & (0.000196) & (0.000193) & (0.000152) & (0.000307) \\
				25$\sim$30℃  & -0.000224*** & -2.06e-05  & -0.000343*** & -0.000185*** & -8.39e-06 \\
				& (5.38e-05)   & (9.46e-05) & (8.84e-05) & (6.74e-05) & (0.000122) \\
				$>$30℃      & 5.79e-05     & -0.000750* & -0.00155*** & -0.000204 & -0.000164 \\
				& (0.000178)   & (0.000436) & (0.000391) & (0.000263) & (0.000586) \\
				wind        & -0.00916***  & -0.00680*** & -0.00507*** & -0.0102*** & -0.00982*** \\
				& (0.000722)   & (0.00130) & (0.00124) & (0.000909) & (0.00146) \\
				sea         & -0.00418***  & 0.00156*** & 0.000678 & -0.00220** & -0.00546* \\
				& (0.000946)   & (0.000602) & (0.000882) & (0.000854) & (0.00323) \\
				visb        & -0.00107     & -0.00152 & -0.00205* & 0.00418*** & 0.00277* \\
				& (0.000672)   & (0.00131) & (0.00113) & (0.000878) & (0.00158) \\
				Constant    & 4.659***     & -1.161* & -0.305 & 2.628*** & 5.882* \\
				& (0.959)      & (0.611) & (0.895) & (0.867) & (3.280) \\
				Controls     & Y & Y & Y & Y & Y \\
				Year FE      & Y & Y & Y & Y & Y \\
				Firm FE      & Y & Y & Y & Y & Y \\
				Observations & 535,067 & 130,288 & 167,440 & 321,108 & 109,152 \\
				R-squared    & 0.193 & 0.155 & 0.191 & 0.180 & 0.109 \\
				\hline
			\end{tabular}
		}
		\caption*{\footnotesize Standard errors in parentheses. *** p$<$0.01, ** p$<$0.05, * p$<$0.1}
	\end{center}
	\vspace{-1em}
\end{table}

%##################################################################################################


\subsection{Benchmarking with Previous Systems}

\vspace{-.2em}
We compare with the leading systems in Table~\ref{tab:system}. We explore various model sizes (see Appendix~\ref{sec:app_details}) and train for 800 epochs.
Similar to autoregressive language models \cite{Brown2020}, we observe encouraging scaling behavior. Further investigation into scaling could be promising.
Regarding metrics, we report 2.35 FID \textit{without} CFG, largely outperforming other token-based methods. Our best entry has 1.55 FID and compares favorably with leading systems. Figure~\ref{fig:results} shows qualitative results.
